Maximizing and Satisficing in Multi-armed Bandits with Graph Information

Pure exploration in multi-armed bandits has emerged as an important framework for modeling decision-making and search under uncertainty. In modern applications, however, one is often faced with a tremendously large number of options. Even obtaining one observation per option may be too costly rendering traditional pure exploration algorithms ineffective. Fortunately, one often has access to similar relationships amongst the options that can be leveraged. In this paper, we consider the pure exploration problem in stochastic multi-armed bandits where the similarities between the arms are captured by a graph and the rewards may be represented as a smooth signal on this graph. In particular, we consider the problem of finding the arm with the maximum reward (i.e., the maximizing problem) or one with a sufficiently high reward (i.e., the satisficing problem) under this model. We propose novel algorithms \textbf{\algoname{}} (GRaph-based UcB) and $\zeta$-\textbf{\algoname{}} for these problems and provide a theoretical characterization of their performance which specifically elicits the benefit of the graph side information. We also prove a lower bound on the data requirement, showing a large class of problems where these algorithms are near-optimal. We complement our theory with experimental results that show the benefit of capitalizing on such side information.

==> Content/Main_Resub_Arxiv/Checklist.tex <==
\section*{Checklist}
% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%
\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper’s contributions and scope?
    \answerYes
    % {See sections \ref{sec:meth}, \ref{sec:theory} and \ref{sec:desp}.}
  \item Did you describe the limitations of your work?
    \answerYes{Please refer to Appendix~\ref{app:broader_impact} for a full discussion.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Please refer to Appendix~\ref{app:broader_impact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}
\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{we include them in the supplementary material.}
\end{enumerate}
\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include the code in supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We specify them in the experiment section~\ref{sec:exp}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}
\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{We did not.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We did not.}
  \item Did you discuss whether and how consent was obtained from people whose data you’re using/curating?
    \answerNo{Data is public.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}
\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}
\end{enumerate}
\newpage{} 
% \section{NeurIPS 2021 Checklist}

% \begin{enumerate}
%     \item \textbf{For all authors..}
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?\\
%   Yes, they do.
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?\\
%   Yes, I have. 
%   \item Did you discuss any potential negative societal impacts of your work?\\
%   Yes we did. Please refer to Appendix~\ref{app:broader_impact}
%   \item Did you describe the limitations of your work?\\
%   Yes we did. Please refer to Appendix~\ref{app:broader_impact} for a full discussion. 
%   \end{enumerate}
%   \item \textbf{If you are including theoretical results...}
%   \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%   \\Yes, we did.
%   \item Did you include complete proofs of all theoretical results?\\
%   Yes, we included them in the supplementary material. 
%   \end{enumerate}
%   \item \textbf{If you ran experiments...}
%   \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?\\
%   We will release the code with the supplementary material. 
%   \item Did you specified all the training details (e.g., data splits, hyperparameters, how they were chosen)?\\
%   Yes we specify them in the experiment section~\ref{sec:exp}
% \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?\\
% We did not report error bars as it is inapplicable to our work.
% \item Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?\\
% Yes. we did. 
%   \end{enumerate}
% %   \item \textbf{If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...}
% %   \begin{enumerate}
% % \item If your work uses existing assets, did you cite the creators?\\
% % Yes we did.
% % \item Did you mention the license of the assets?\\
% % No we did not. 
% % \item Did you include any new assets either in the supplemental material or as a URL?\\
% % No we did not. 
% % \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?\\
% % No we did not. 
% % \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?\\
% % No we did not.
% % \end{enumerate}
% %   \item \textbf{If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...}
% %   Not applicable
  
% \end{enumerate}

==> Content/Main_Resub_Arxiv/alternate_lower_bounds.tex <==
\color{purple}
\section{Lower Bounds}
Let us consider an $n$-armed bandit setup with arm indices $[1, \dots, n]$. Let $\mu^*$ indicate the mean of the optimal arm and $\mu_i$ indicate the mean values of all other arms such that $\mu_i < \mu^*$. For the rest of this section, without loss of generality, let the index of optimal arm be 1. 

% Given any graph $H$, let $\mathcal{C}_H$ denote the set of sets of indices in the same cluster in $H$, i.e. if $C_H\in \mathcal{C}_H$ then there $i$ and $j$ are connected in $H$, $\forall i, j\in C_H$. It is worth noting that $|\mathcal{C}_H|$ denotes the number of clusters in $H$. Let $C_H(i)$ denote the set of indices in $\mathcal{C}_H$ corresponding to the cluster with arm $i$. 
\begin{definition}[$(\epsilon, \delta)$-PAC]
An algorithm is $(\epsilon, \delta)$-PAC for a multi-armed bandit problem with sample complexity $T$, if it outputs an $\epsilon$-optimal arm, $a'$, with probability at-least $1-\delta$, when it terminates, and the number of time steps the algorithm performs until it terminates is bounded by $T$. 
\end{definition}

\begin{remark}
Any $(\epsilon, \delta)$-PAC algorithm can terminate before $T$ time steps have passed. The sample complexity considered here is the complexity of the worst trajectory
\end{remark}

The complexity for solving the vanilla $n$-armed bandit problem was proved in~\cite{mannor2004sample} where, for any $\delta$-PAC algorithm, the necessary number of samples scales as,
\begin{align}\label{eq:vanilla-bandit-complexity}
    T_{\text{necessary}} \geq \sum_{i\neq i^*} \frac{\log\delta^{-1}}{\Delta_i^2}
\end{align}
where $i^*$ is the arm with the optimal mean. 

\subsection{Graph information}
Taking it further from~\eqref{eq:vanilla-bandit-complexity}, in the presence of side information the lower bounds can be taken further down because of more information. Next we focus on the following questions : 1) Can we establish lower bounds which reflect the availability of this side information? 2) Are the lower bounds tight enough to be achieved by any algorithm?

\subsection{Perfect graph information}
In the presence of perfect graph we can establish the following lower bounds, 
\begin{theorem}\label{thm:lower-bound-perfect-graph}
Given an $n$-armed bandit model with associated mean vector $\pmb{\mu}\in \mathbb{R}^n$ and similarity graph $G$ with edge set $E_G$ such that $\mu_i = \mu_j~~\forall (i, j)\in E_G$. Define
\begin{align}
    T_{\text{necessary}}\geq \sum_{C\in \mathcal{C}_G} \max_{j\in C}\left\{ \frac{4\sigma^2}{\Delta_j^2}\log{\left(\frac{1}{2\delta}\right)}\right\}
\end{align}
Then any $\delta$-PAC algorithm will need atleast $T_{\text{necessary}}$ steps to terminate, provided $\delta \leq 0.15$ and the optimal arm isolated in graph $G$
\end{theorem}
The condition of isolated optimal arm in graph $G$ with the perfect graph information is crucial. If not, then there is an arm $i$ which is not the optimal arm such that $\mu_i = \mu^*$ (since there is an edge with the optimal arm and arm $i$), which violates the uniqueness of optimal arm. 
 
\subsection{Imperfect graph information}
Assuming the availability of a \textit{similarity graph} $G$ which is smooth on the mean vector, i.e. $\langle \pmb{\mu}, G\pmb{\mu}\rangle\leq \epsilon$ for some $\epsilon>0$, the necessary number of samples required for any $\delta$-PAC algorithm for:

\begin{theorem}\label{thm:lower-bound}
Given an $n$-armed bandit model with associated mean vector $\pmb{\mu}\in \mathbb{R}^n$ and similarity graph $G$ smooth on $\pmb{\mu}$, i.e. $\langle\pmb{\mu}, L_G\pmb{\mu}\rangle \leq \epsilon$, $\epsilon> 0$ and subgraph $F$ be constructed from $G$ by removing the optimal arm (arm 1 in this case) from the rest of the graph. Define
\begin{align}
    T_{\text{necessary}}
    % &\ \geq \sum_{C\in \mathcal{C}_F}\max_{j\in C} \left\{\frac{4\sigma^2}{\Delta_j^2}\log{\left(\frac{|\mathcal{C}_F|}{2\delta}\right)}\right\}\nonumber\\
    &\ \geq \sum_{C\in \mathcal{C}_F/ \mathcal{C}_G}\max_{j\in C} \left\{\frac{4\sigma^2}{\Delta_j^2}\log{\left(\frac{1}{2\delta}\right)}\right\}\nonumber\\
    &\ + \sum_{i \in \mathcal{H}} \frac{4\sigma^2}{(\Delta_j + \epsilon)^2}\log{\left(\frac{1}{2\delta}\right)}\nonumber\\
    &\ +\sum_{C\in \mathcal{C}_F\cap \mathcal{C}_G}\max_{j\in C} \left\{\frac{4\sigma^2}{\Delta_j^2}\log{\left(\frac{1}{2\delta}\right)}\right\}
\end{align}
where $\mathcal{H} = \{i ~|~ \Delta_i < \epsilon\}$. Then any $\delta$-PAC algorithm will need atleast $T_{\text{necessary}}$ steps to terminate, provided $\delta \leq 0.15$. 
\end{theorem}
% \textit{Proof sketch for Theorem~\ref{thm:lower-bound}:}

% The central idea of the proof is to construct a subproblem of the original $n$-armed bandit problem and obtain lower bounds by obtaining lower bounds for the subproblem. To that end, construct subgraph $F$ from $G$ by removing all the links of optimal arm (arm 1 in this case) from the rest of the graph. Further, construct a subproblem of the $n$-armed bandit setup by picking the arm with highest mean from each connected component $\mathcal{C}_F$. and $\mathcal{A}$ be the set of indices of arms with the maximum means in their individual clusters, i.e. $|\mathcal{A}\cap C|=1~~~\forall C\in \mathcal{C}_F$ and $\mu_{\mathcal{A}\cap C} = \max\{\mu_i| i\in C\}~~~\forall C\in \mathcal{C}_F$. Now consider this new $|\mathcal{C}_F|$-armed bandit problem with $\mathcal{A}$ as the arms. Observe that the sample complexity of solving the new $|\mathcal{C}_F|$-armed bandit subproblem is smaller than that of solving the original $n$-armed bandit problem.

% \subsubsection{Comparison of the sample complexity in Theorem~\ref{thm: sample_complexity} to lower bounds in Theorem~\ref{thm:lower-bound}}

With the freedom of choice of the mean distribution of all the arms $\{\mu_i\}_{i=1}^n$, the side information graph $G$ and the violation constant $\epsilon$, it is hard to compare the exact nature of the gap between the upper (Theorem~\ref{thm: sample_complexity}) and lower bound (Theorem~\ref{thm:lower-bound}). Even with the difficulty, we show that for a wide variety of problem setups the upperbound on the sample complexity provided in Theorem~\ref{thm: sample_complexity} matches the lower bound established in Theorem~\ref{thm:lower-bound} in $\Delta_i := \mu^* - \mu_i$ upto a constant factor.

The lower bound on sample complexity depends on the structure of the side-information graph $G$, while rest of the systems parameters $(\{\mu_i\}_{i=1}^n, \epsilon)$ are kept constant. We show the variation in the expression of Theorem~\ref{thm:lower-bound} with changing structure on graph $G$ as follows:  
\begin{corollary}[Star graph]\label{cor:lower-bounds-star}
Consider the setup as in Theorem~\ref{thm:lower-bound} with the further restriction that $G$ is a star graph with the central node as the optimal arm. Define,
\begin{align}
    T_{\text{necessary}}\geq \sum_{i=2}^n \frac{4\sigma^2}{\epsilon}\log{\left(\frac{n-1}{2\delta}\right)}
\end{align}
Then any $\delta$-PAC algorithm will need atleast $T_{\text{necessary}}$ steps to terminate, provided $\delta \leq 0.15$. 
\end{corollary}
% This matches the upperbound established in Theorem~\ref{thm: sample_complexity} under similar setup conditions. 

\begin{corollary}[Isolated clusters]\label{cor:lower-bounds-clusters}
Consider the setup as in Theorem~\ref{thm:lower-bound} with the further restriction that graph $G$ be such that the optimal node is isolated and arms $[2, \dots, n]$ are split in $k$ clusters. Define,
\begin{align}
    T_{\text{necessary}}\geq \sum_{C\in \mathcal{C}_G} \max_{j\in C}\left\{ \frac{4\sigma^2}{\Delta_j^2}\log{\left(\frac{|C_G|}{2\delta}\right)}\right\}
\end{align}
Then any $\delta$-PAC algorithm will need atleast $T_{\text{necessary}}$ steps to terminate, provided $\delta \leq 0.15$. 
\end{corollary}

As can be seen in Corollary~\ref{cor:lower-bounds-star} and~\ref{cor:lower-bounds-clusters}, the lower bound expression can scale as standard $n$-armed bandit (implying no added advantage of having graph side-information) or can be have as $|\mathcal{C}_G|$-bandit problem (scales as the number of clusters in graph G rather than number of nodes $n$) purely by changing the similarity graph $G$. The difference between $\mathcal{C}_F$ and $\mathcal{C}_G$ can lead to more interesting behaviour in terms of lower bound expressions on sample complexity. 

% Note that in Corollary~\ref{cor:lower-bounds-star} the lower bound has summation over all the suboptimal arms $[2, \dots, n]$ where-else Corollary~\ref{cor:lower-bounds-clusters} only sums over the total number of clusters. In the next section, we leverage the graph side information to device an algorithm which provably reaches improves the sample complexity than vanilla best arm identification algorithms.  

% Since the statement of sample complexity caters to a much larger class of bandit setups than used to prove Theorem~\ref{thm:minimax_subclass} ($\pmb{\mu}\in \mathbb{R}^n$ and $\langle\mu, L_G\mu\rangle \leq \epsilon$ as opposed to the restrictive $\langle\mu, L_G\mu\rangle = 0$), the lower bound  calculations are expected to become more complicated.


Further note that, 
\begin{remark}\label{rem:blow-up}
Provided the setup of Theorem~\ref{thm:lower-bound}, then no $\delta$-PAC algorithm can solve \textit{P1} if $\epsilon\rightarrow 0$ and $ d(1) >0$, where $d(\cdot)$ indicates the degree of the vertex. 
\end{remark}
This behaviour of Theorem~\ref{thm:lower-bound} is expected. Notice that $|\mathcal{C}_F/\mathcal{C}_G| =0$ if and only if optimal arm was isolated in similarity graph $G$. Hence graph $G$ consisting of an edge involving the optimal arm and $\epsilon \rightarrow 0$ implies existence of another arm with exact same mean as the optimal arm, which violates the uniqueness of optimal arm required to solve \textit{P1}. 

In the further text, we remove this uniqueness assumption on optimal arm in the Section~\ref{sec:zeta_best_arm}.

% Note that the lower bound in Theorem~\ref{thm:lower-bound} scales as $O\left(\frac{|\mathcal{C}_F/\mathcal{C}_G|}{\epsilon}\right)$. Thus, $T_{\text{necessary}}$ blows up as $\epsilon \rightarrow 0$ if $|\mathcal{C}_F/\mathcal{C}_G| > 0$. 

\color{black}



==> Content/Main_Resub_Arxiv/conclusion.tex <==
% \section{Conclusion}\label{sec:conc}
% In this work, we propose a novel algorithm \algoname{} for best arm identification in the presence of graph information. We provide a sample complexity bound on the performance of \algoname, and show that by utilizing  graph side information, we can obtain the best arm significantly faster. We also provided the sample complexities to obtain an approximate optimal arm. Experiments show. 


\begin{comment}


\nr{do we need all these?(space constraint)}
\begin{enumerate}
    \item \textbf{Limitation}
    \item \textbf{Computational overload}
Including graph makes it a computationally heavy framework. Making the algorithm distributed in nature to make it a computationally inexpensive is potential future problem in consideration, but is out of scope of this work. 
    \item \textbf{Violation of gaussian noise}
    \item \textbf{Violation of graph smoothness}
    \item \textbf{Experimental shortcomings}
\end{enumerate}

\section{Broader impact}
Our method can be used for various applications, such as drug discovery, advertising and recommendation systems. As such, our method finds practical use in crucial applications such as the fight against infectious diseases, as well as those that generate revenue to large corporations. Hub nodes in the graph have a stronger likelihood of being picked as the best arm, which can lead to a ``rich get richer" phenomenon. Incorporating fairness constraints, or subsampling the edges from popular nodes will help mitigate this. In applications such as drug discovery, designing the rewards becomes vital, since the best arm (and $\zeta-$ best arm) heavily depend on the reward. 

\end{comment}

==> Content/Main_Resub_Arxiv/contributions.tex <==
\begin{comment}
We consider the classical multi-armed bandit problem, but with additional information on the expected rewards between the arms in form of a graph. To start with, rather than looking at the expected regret,  we develop PAC style bounds on the error probability of missing the best arm identification. The agent’s goal is to find,  with high probability,  a near optimal arm, namely, with probability at least 1-$\delta$ output an $\epsilon$-optimal arm. This naturally abstracts the case where the agent needs to choose one specific arm, and it is given only limited exploration initially.  Our main complexity criterion, in addition to correctness, is the number of steps taken by the algorithm,  which can be viewed as pure exploration steps. We give the first closed form sample complexity bounds incorporating graphs for the best arm identification process with high probability. ~\citep{kocak2020best} analyses similar problem to ours, but does not provide a closed for solution or any insights as our work. This work is in contrast to many other results for the multi-armed bandit problem using graphs~\citep{valko2014spectral, yang2020laplacianregularized}, where the main aim is to maximize the expected cumulative reward while both exploring and exploiting. 

\com{Transient information utilization}
The core principle which we are following in this paper is use side information as a tool to "quickly" sift through suboptimal arms while also making sure no underlying assumption on the mean distribution is implemented (unlike linear bandits). This enables the focus of data gathering resources more on "good" arms or churn out a relatively good arm faster. In accordance to this view, we use the side information in a transient fashion. Transient in the sense that the impact of the side information is really high when the data gathering is during its initial stages and fades off to resemble vanilla best arm identification as more and more data is gathered. 

There are several benefits of using the "transient" approach. Firstly, unlike in linear bandits, there is no strict assumption on the underlying model on $\pmb{\mu}$. Secondly, because of the transient nature of the usage of side information, this approach could potentially be used along side any other strict model assumptions on the mean vector $\pmb{\mu}$. For e.g. the current analysis can be extended to case of best arm identification with linear bandits modelling.

\com{Imperfect knowledge utilization + Perfect information leads to a stronger sample complexity}
Transient nature of the information we use couples really well with \textit{approximate} side information. In this write-up this side information is in form of graphs implying that the data need not be completely accurate (the precise statement to appear later in text). Apart for showing analysis for \textit{approximate} side information, we also prove that given \textit{perfect} information leads to stronger sample complexity bounds than in the case of best arm identification without graph information. 

\com{Quick removals}
One of the most promising outcomes of using the side information is the "quick" removal of suboptimal arms. More concretely, by sampling few of the arms in tightly connected clusters, we can eliminate clusters of arms as being sub-optimal because of the side information. This kind of result is what is precisely expected for high frequency application with huge data gathering mechanisms like ads-placement, etc.  

\com{No dependence on $\lambda$}
One of the key requirements in previous results in graph bandits is the permanent addition of $\lambda$ times identity matrix to the counting matrix (more on this terminology later). This addition ultimately becomes a dominant factor in the analysis and shows up the sample complexity bounds. 

We show that this is unnecessary and the semi-definiteness of the system is precisely how we can take advantage of the clustered nature of the graph to provide better sample complexity arguments. 

\com{No time dependent "effective" dimension}
\pk{need better argument} Unlike~\citep{valko2014spectral} we dont need a horizon dependent notion to make our bounds work. The bounds depend on the mean distribution and graph properties. 


\com{Asking different question}
The results from using graph side infomration are more imapctful if we ask the question as follows \begin{align}
    \text{How to quickly get rid of suboptimal arms}
\end{align}
Another way of asking the same question is 
\begin{align}
    \text{How to quickly reach the set of "good" arms}
\end{align}
which is a question of dire importance to many real world applications. We show that usage of graph side information provides quite an edge in such cases. 

\end{comment}

==> Content/Main_Resub_Arxiv/difference_linear_bandits.tex <==
\section{Comparison between  structural bandits}\label{sec:graph_vs_linear}
In this section, we show theoretically and intuitively, the difference between the framework of graph bandit and that of  linear bandits. Bandits with graph side-information reduces the complexity of solving the classic best-arm identification problem (this could be quite hard when the number of arms blows up!) using similarity graph networks wherelse, linear bandits assumes a lower-dimensional representation of arm rewards. Formally stating the two setups:
\begin{itemize}
\item{\bf (a) Linear bandits}

Consider an $n$-armed linear bandit problem, where each arm $i\in [n]$ is associated with a feature vector $\mathbf{x}_i\in \mathbb{R}^d$, where $d$ can be lower than $n$. In each round $t$, the learner chooses an action $\textbf{a}_t = \mathbf{x}_i$ for some $i\in [n]$ and observes the reward $y_t = \langle \mathbf{a}_t, \pmb{\theta}\rangle + \eta_t$, where $\pmb{\theta}\in \mathbb{R}^d$ is an unknown reward vector and the $\eta_t$ is a subgaussian random noise with $\sigma^2$ variance.

\item{\bf (b) Bandits with graph side information}

Consider an $n$-armed linear bandit problem parameterized by mean vector $\mathbf{\mu}\in \mathbb{R}^n$, where $\mu_i$ corresponds to the mean value of arm $i$. Additional information is provided using graph $G$ such that $\langle \pmb{\mu}, L_G\pmb{\mu}\rangle \leq \epsilon$, where $\epsilon>0$. In each round $t$, the learner chooses some arm $i\in [n]$ and observes the reward $y_t = \mu_i + \eta_t$, where $\eta_t$ is a subgaussian random noise with $\sigma^2$ variance.
% Consider $n$-armed bandit problem with similarity side-information in the presence of graph $G$ such that $$\langle \pmb{\mu}, L_G\pmb{\mu}\rangle \leq \epsilon,$$ where $\epsilon >0$ and $L_G$ is the Laplacian matrix corresponds to graph $G$. 
% Consider $n$-armed linear bandits setup, where each arm corresponds to some linear vector/context $\mathbf{a}_i\in \mathbb{R}^d$ for some $d< n$. The linear model assumption is that,
% \begin{align}
%     \exists~ \pmb{\theta}^*\in \mathbb{R}^n \text{ such that }\mu_i = \langle\mathbf{a}_i, \pmb{\theta}^*\rangle~~~i =1,2,3\nonumber
% \end{align}

% Further, we show a small toy example to intuitively motivate the difference between the aforementioned two setups
\end{itemize}

In both these setups, aim is to detect the arm with the best mean reward, i.e. detect $i^* = \mathop{\arg\max}_{i\in[n]} \mu_i$. To get an intuitive understanding of the difference between the two frameworks mentioned, consider the following toy example: Consider a $3$-armed bandit setup parametrized by mean vector $\pmb{\mu}\in \mathbb{R}^3$. We analyse the best arm-identification problem for the following two cases of additional structure:

\begin{itemize}
    \item {\bf (a) $3$-{armed linear bandits}} : Consider three feature vectors $\{\mathbf{a}_1,\mathbf{a}_2, \mathbf{a}_3\}\in \mathbb{R}^2$ corresponding to the three arms. Let  $\exists~\theta^* \in \mathbb{R}^2$ indicate the underlying reward vector such that $
    \mu_i = \langle\mathbf{a}_i, \pmb{\theta}^*\rangle~~~i =1,2,3$. 
Without loss of generality assume that \begin{align}\label{eq:toy_linear_vector}
    \mathbf{a}_1  = \mathbf{e}_1,~~
    \mathbf{a}_2  = a\mathbf{e}_1 + b\mathbf{e}_2, ~~
    \mathbf{a}_3  = c\mathbf{e}_1 + d\mathbf{e}_2
\end{align} where $\mathbf{e}_{1,2}$ indicate the canonical basis of $\mathbb{R}^2$ and $a,b,c,d\in \mathbb{R}$ indicates some constants such that $b\neq 0$ (we are requiring this condition to ensure full span). Thus we can definitely say that, $\mu_3 = c\mu_1 + \frac{d}{b}\left(\mu_2 - a\mu_1\right)$ concluding that exact information of $\mu_1, \mu_2$ and constants $a,b,c,d$ leads to complete estimation of $\mu_3$. 

\item{\bf (b) $3$-{armed bandit problem with graph side information}} : Let a given graph $G$ encodes the similarity relation between the mean values of the three arms, i.e. $\langle \pmb{\mu}, L_G\pmb{\mu}\rangle \leq \epsilon$ for some constant $\epsilon > 0$. Let $E_G$ denote the edge set of graph $G$ and $\mathbbm{1}_{(1,2)}, \mathbbm{1}_{(2,3)}$ and $\mathbbm{1}_{(1,3)}$ encodes the event if edges $\{(1,2), (2.3), (1,3)\}\in E_G$ are present in graph $G$. The graph structure can thus be represented as,
\begin{align}\label{eq:eps_big}
    \mathbbm{1}_{(1,2)}(\mu_1-\mu_2)^2 + \mathbbm{1}_{(2,3)}(\mu_2-\mu_3)^2 + 
    \mathbbm{1}_{(1,3)}(\mu_1-\mu_3)^2 \leq \epsilon
\end{align}

Take the simple case of edge $(2,3)$ being present and $(1,3)$ absent, then following holds true,
\begin{align}
    \mu_{\text{low}} := \mu_2 - \sqrt{\epsilon - \mathbbm{1}_{(1,2)}(\mu_1 - \mu_2)^2}\leq \mu_3 \leq \mu_2 + \sqrt{\epsilon - \mathbbm{1}_{(1,2)}(\mu_1 - \mu_2)^2} := \mu_{\text{high}}\nonumber
\end{align}
Even with the complete knowledge of $\mu_1, \mu_2$ and other system parameters, one can only estimate $\mu_3$ upto an interval $[\mu_{\text{low}}, \mu_{\text{high}}]$. 
\end{itemize}
In conclusion, with the linear bandit model $\mu_3$ could be determined by knowledge of $\mu_1, \mu_2$ wherelse in the graph bandit framework, knowledge of $\mu_1, \mu_2$ is insufficient to determine $\mu_3$, making the graph bandit framework much more difficult to tackle. We solidify intuition developed so far in the following result. 

\begin{proposition}\label{prop:graph_vs_linear_thm}
Consider $n$-armed bandit setup parameterized by mean vector $\pmb{\mu}\in \mathbb{R}^n$. Given graph $G$ and $\epsilon >0$, let $D_{G, \epsilon} := \{\pmb{\mu}\in \mathbb{R}^n |~~ \langle \pmb{\mu}, L_G\pmb{\mu}\rangle \leq \epsilon\}$ represent a subset of bandit problems in $\mathbb{R}^n$,  $L_G$ denoting the laplacian matrix corresponding to graph $G$. Then $m(D_{G, \epsilon})>0$ where $m(\cdot)$ is the Lebesgue measure on $\mathbb{R}^n$.
\end{proposition}

Proposition~\ref{prop:graph_vs_linear_thm} lists that given a graph $G$ and $\epsilon>0$, the set of problems which can be encompassed by the graph bandit framework is a positive measure set. This is in direct contradiction to the zero measure set described through linear bandit setup. This makes tackling graph-bandit framework harder. In this paper, we not only propose \algoname{}, but also prove the theoritical guarantees behind the same. The detailed discussion of the toy example and full proof of Proposition~\ref{prop:graph_vs_linear_thm} can be obtained in Appendix~\ref{app:as_linear_bandit}.

==> Content/Main_Resub_Arxiv/discussion_limitation.tex <==
\section{Conclusion}\label{app:broader_impact}

In this work, we consider the problem of best arm identification (and approximate best arm identification) when one has access to information about the similarity between the arms in the form of a graph. We propose a novel algorithm \algoname{} for this important family of problems and establish sample complexity guarantees for the same. In particular, our theory explicitly demonstrated that benefit of this side information (in terms of the properties of the graph) in quickly locating the best or approximate best arms. We support these theoretical findings with experimental results in both simulated and real settings. 

{\bf Future Work and Limitations. }
We outline several sampling policies inspired by our theory in Section~\ref{sec:exp}; an extension of our theoretical results to account for these improved sampling policies is a natural candidate for further exploration. The algorithms and theory of this paper assume knowledge of (an upper bound) on the smoothness of the reward vector with respect to the graph. While this is where one uses domain expertise, this could be hard to estimate in certain real world problems. A generalization of the algorithmic and theoretical framework proposed here that is \emph{adaptive} to the unknown graph-smoothness is an exciting avenue for future work\footnote{T. Tony Cai, Ming Yuan "Adaptive covariance matrix estimation through block thresholding," The Annals of Statistics, Ann. Statist. 40(4), 2014-2042, (August 2012)}$^,$\footnote{Banerjee, T., Mukherjee, G., \& Sun, W. (2020). Adaptive sparse estimation with side information. Journal of the American Statistical Association, 115(532), 2053-2067.}. The sub-Gaussianity assumption of this work can also be generalized to other tail behaviors in follow up work. Another limitation of this work is that the statistical benefit of the graph-based quadratic penalization comes at a computational cost -- each mean estimation step involves the inversion of an $n\times n$ matrix which has a complexity of $O(n^2\log(n))$. However, an exciting recent line of work suggests that this matrix inversion can be made significantly faster when coupled with a spectral sparsification of the graph $G$\footnote{Spielman, D. A., \& Teng, S. H. (2011). Spectral sparsification of graphs. SIAM Journal on Computing, 40(4), 981-1025.}$^,$\footnote{Vishnoi, Nisheeth K. "Lx= b." Foundations and Trends in Theoretical Computer Science 8.1–2 (2013): 1-141.} while controlling the statistical impact of such a modification. In the context of this problem, this suggests a compelling avenue for future work that studies the statstics-vs-computation tradeoffs in using graph side information.  

% One of our major assumptions is the existence and knowledge of $\epsilon >0$ such that $\langle\pmb{\mu}, L_G\pmb{\mu}\rangle$ where $\pmb{\mu}$ is the mean vector and $G$ is the given similarity graph. 

For this work, we demonstrated the advantages of this side information in pure exploration problems, given knowledge of such an $\epsilon$. Extensions that consider goodness-of-fit and misspecification with respect to the graph $G$ and smoothness parameters $\epsilon$ are interesting avenues for follow up work. Finally, we focus on the ridge-type regularizer of the form $\langle\mathbf{\mu}, L_G\mathbf{\mu}\rangle$. For future work, it may be productive to expand to a much broader class of regularizers such as those of the form of $\|A\mathbf{\mu}\|^p_q$, where $A$ represents a information/ structural constraint matrix and $p,q$ are some positive  numbers. 
% \begin{enumerate}
%     \item \textbf{Limitation}
%     \item \textbf{Computational overload}
% Including graph makes it a computationally heavy framework. Making the algorithm distributed in nature to make it a computationally inexpensive is potential future problem in consideration, but is out of scope of this work. 
%     \item \textbf{Violation of subgaussian noise}
%     \item \textbf{Violation of graph smoothness}
%     \item \textbf{Experimental shortcomings}
% \end{enumerate}

% \subsection{Broader impact}
{\bf Potential Negative Social Impacts. }Our methods can be used for various applications such as drug discovery, advertising, and recommendation systems. In scientifically and medically critical applications, the design of the reward function becomes vital as this can have a significant impact on the output of the algorithm. One must take appropriate measures to ensure a fair and transparent outcome for various downstream stakeholders. With respect to applications in recommendation and targeted advertising systems, it is becoming increasingly evident that such systems may exacerbate polarization and the creation of filter-bubbles. Especially the techniques proposed in this paper could reinforce emerging polarization (which would correspond to more clustered graphs and therefore better recommendation performance) when used in such contexts. It will of course be of significant interest to mitigate such adverse outcomes by well-designed interventions  or by considering multiple similarity graphs that capture various dimensions of similarity. This is a compelling avenue for future work. 

% As such, our method finds practical use in crucial applications such as the fight against infectious diseases, as well as those that generate revenue to large corporations. Hub nodes in the graph have a stronger likelihood of being picked as the best arm, which can lead to a ``rich get richer" phenomenon. Incorporating fairness constraints, or subsampling the edges from popular nodes will help mitigate this. In applications such as drug discovery, designing the rewards becomes vital, since the best arm (and $\zeta-$ best arm) heavily depend on the reward. 


% (We should add some )
% While the problem of including side information into sampling procedure is very broad, we are targeting one part of the problem of having graph side information, specifically of the form $\langle\mathbf{\mu}, L_G\mathbf{\mu}\rangle \leq \epsilon$. The following are noteworthy points :
% \begin{itemize}
%     \item Generalizing the results to a broader class of side information is a very interesting topic for further work.
%     \item Goodness of fit w.r.t $\epsilon$: Providing theoretical analysis for misspecification of $\epsilon$ and algorithmic additions to avoid the same is beyond the scope of the paper. A promising method for doing this is a appropriate decay scheme. 
%     \item TODO : Not able to think around the restrictions on the scaling of $\epsilon$ with $t$ and $n$ and other system parameters. 
% \end{itemize}

==> Content/Main_Resub_Arxiv/graph_vs_linear.tex <==
\section{Bandits with structure}\label{sec:graph_vs_linear}

The problems of solving bandits with graph side-information provides one source of information to sift through the arms in order to reduce the complexity of solving the classic best-arm identification problem (this could be quite hard when the number of arms blows up!). The graph information is in the form of the Laplacian matrix $L_G$ which motivates the comparison of the graph bandit setup to linear bandits. It remains to be answered whether one class of problems discussed here is completely subsumed by another or vice-versa. In this section we argue that the two setups: bandits with graph side-information and linear bandits are fundamentally different. We first motivate this difference by providing a toy example and then solidifying it using measure theoretic arguments.

Formally stating the two setups:
\begin{itemize}
\item{\bf (a) Linear bandits}

Consider an $n$-armed linear bandit problem, each arm $i\in [n]$ is associated with a feature vector $\mathbf{x}_i\in \mathbb{R}^d$, where $d$ can be lower than $n$. In each round $t$, the learner chooses an action $\textbf{a}_t = \mathbf{x}_i$ for some $i\in [n]$ and observes the reward $y_t = \langle \mathbf{a}_t, \pmb{\theta}\rangle + \eta_t$, where $\pmb{\theta}\in \mathbb{R}^d$ is an unknown parameter and the $\eta_t$ is a subgaussian random noise with $\sigma^2$ variance. Denote the arm with the best mean reward with $i^*$, i.e. $i^* = \mathop{\arg\max}_{i\in[n]} \langle \mathbf{x}_i, \pmb{\theta}\rangle$.

\item{\bf (b) Bandits with graph side information}

Consider an $n$-armed linear bandit problem, each arm $i\in [n]$ is associated with a mean vector $\mathbf{\mu}\in \mathbb{R}^n$, where $\mu_i$ corresponds to the mean value of arm $i$. We are provided with further information using a graph $G$ that $\langle \pmb{\mu}, L_G\pmb{\mu}\rangle \leq \epsilon$, where $\epsilon>0$. In each round $t$, the learner chooses some arm $i\in [n]$ and observes the reward $y_t = \mu_i + \eta_t$, where $\eta_t$ is a subgaussian random noise with $\sigma^2$ variance. 

% Consider $n$-armed bandit problem with similarity side-information in the presence of graph $G$ such that $$\langle \pmb{\mu}, L_G\pmb{\mu}\rangle \leq \epsilon,$$ where $\epsilon >0$ and $L_G$ is the Laplacian matrix corresponds to graph $G$. 
% Consider $n$-armed linear bandits setup, where each arm corresponds to some linear vector/context $\mathbf{a}_i\in \mathbb{R}^d$ for some $d< n$. The linear model assumption is that,
% \begin{align}
%     \exists~ \pmb{\theta}^*\in \mathbb{R}^n \text{ such that }\mu_i = \langle\mathbf{a}_i, \pmb{\theta}^*\rangle~~~i =1,2,3\nonumber
% \end{align}

% Further, we show a small toy example to intuitively motivate the difference between the aforementioned two setups
\end{itemize}

In both these setups, denote the arm with the best mean reward with $i^*$, i.e. $i^* = \mathop{\arg\max}_{i\in[n]} \mu_i$. The goal of the learner is to output the index of the arm $i^*$ with probability $1-\delta$, $\delta>0$ in as few samples as possible. 

\subsection{Toy example}\label{subsec:toy}
Consider a $3$-armed bandit setup with mean value $\{\mu_i\}_{i=1}^3$. We analyse the best arm-identification problem for the two cases of:

\begin{itemize}
    \item {\bf (a) $3$-{armed linear bandits}} : Consider three feature vectors $\{\mathbf{a}_1,\mathbf{a}_2, \mathbf{a}_3\}\in \mathbb{R}^2$ corresponding to the three arms. Then the linear model assumption would indicate that $\exists~\theta^* \in \mathbb{R}^2$ such that:
\begin{align}\label{eq:toy_linear_mean}
    \mu_i = \langle\mathbf{a}_i, \pmb{\theta}^*\rangle~~~i =1,2,3
\end{align}
Without loss of generality assume that \begin{align}\label{eq:toy_linear_vector}
    \mathbf{a}_1 &\ = \mathbf{e}_1, \nonumber\\ 
    \mathbf{a}_2 &\ = a\mathbf{e}_1 + b\mathbf{e}_2, \nonumber\\ 
    \mathbf{a}_3 &\ = c\mathbf{e}_1 + d\mathbf{e}_2
\end{align}  where $\mathbf{e}_{1,2}$ indicate the canonical basis of $\mathbb{R}^2$ and $a,b,c,d\in \mathbb{R}$ indicates some constants such that $b\neq 0$ (we are requiring this condition only to ensure that $\mathbf{a}_1$ does not align with $\mathbf{a}_2$). 

Merging the knowledge of equations~\eqref{eq:toy_linear_mean} and~\eqref{eq:toy_linear_vector}, we can obtain the following equation,
\begin{align}
    \mu_3 = c\mu_1 + \frac{d}{b}\left(\mu_2 - a\mu_1\right)
\end{align}
concluding that exact information of $\mu_1, \mu_2$ leads to full estimation of $\mu_3$. We compare this dependence behaviour of $\mu_3$ on $\mu_1, \mu_2$ in linear bandit model with graph side information model. 

\item{\bf (b) $3$-{armed bandit problem with graph side information}} : Let graph $G$ encodes the similarity relation between the mean values of the three arms, i.e. \begin{align}\label{eq:toy_graph}
    \langle \pmb{\mu}, L_G\pmb{\mu}\rangle \leq \epsilon
\end{align} for some constant $\epsilon > 0$. Let $E_G$ denote the edge set of graph $G$ and $\mathbbm{1}_{(1,2)}, \mathbbm{1}_{(2,3)}$ and $\mathbbm{1}_{(1,3)}$ encodes the event if edges $\{(1,2), (2.3), (1,3)\}\in E_G$ are present in graph $G$. For the sake of a non-trivial analysis we take that either $(1,3)$ or $(2,3)$ is present in $E_G$ (alternate case is argued later). 

We can write equation~\eqref{eq:toy_graph} as,
\begin{align}\label{eq:eps_big}
    \mathbbm{1}_{(1,2)}(\mu_1-\mu_2)^2 + \mathbbm{1}_{(2,3)}(\mu_2-\mu_3)^2 + 
    \mathbbm{1}_{(1,3)}(\mu_1-\mu_3)^2 \leq \epsilon
\end{align}
In order to compare the dependence behaviour of $\mu_3$ on $\mu_1, \mu_2$ we can rearrange the above as,
\begin{align}\label{eq:mu3_quadratic}
    &\ \mu_3^2 \left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right) -2\mu_3\left(\mathbbm{1}_{(2,3)}\mu_2 + 
    \mathbbm{1}_{(1,3)}\mu_1\right) \nonumber\\ &\ + \left(\mathbbm{1}_{(2,3)}\mu_2^2 + 
    \mathbbm{1}_{(1,3)}\mu_1^2 + \mathbbm{1}_a(\mu_1-\mu_2)^2 - \epsilon\right) \leq 0
\end{align}
Looking at equation~\eqref{eq:mu3_quadratic} as a quadratic in $\mu_3$ and finding the solutions, we obtain that,
\begin{align}
    &\ \mu_3\geq \frac{\left(\mathbbm{1}_{(2,3)}\mu_2 + 
    \mathbbm{1}_{(1,3)}\mu_1\right) }{\left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right)}\nonumber\\
    &\ - \frac{ \sqrt{\left(\mathbbm{1}_{(2,3)}\mu_2 + 
    \mathbbm{1}_{(1,3)}\mu_1\right)^2 - \left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right)\left(\mathbbm{1}_{(2,3)}\mu_2^2 + 
    \mathbbm{1}_{(1,3)}\mu_1^2 + \mathbbm{1}_{(1,2)}(\mu_1-\mu_2)^2 - \epsilon\right) }}{\left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right)}\nonumber\\
    &\ \mu_3\leq \frac{\left(\mathbbm{1}_{(2,3)}\mu_2 + 
    \mathbbm{1}_{(1,3)}\mu_1\right) }{\left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right)}\nonumber\\
    &\ + \frac{ \sqrt{\left(\mathbbm{1}_{(2,3)}\mu_2 + 
    \mathbbm{1}_{(1,3)}\mu_1\right)^2 - \left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right)\left(\mathbbm{1}_{(2,3)}\mu_2^2 + 
    \mathbbm{1}_{(1,3)}\mu_1^2 + \mathbbm{1}_{(1,2)}(\mu_1-\mu_2)^2 - \epsilon\right) }}{\left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right)}\nonumber\\
\end{align}

Further simplifying it, we get the following:
\begin{align}\label{eq:bounds_simplified}
    &\ \mu_3\geq \frac{\left(\mathbbm{1}_{(2,3)}\mu_2 + 
    \mathbbm{1}_{(1,3)}\mu_1\right) }{\left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right)}\nonumber\\
    &\ -\frac{ \sqrt{\epsilon\left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right) - \mathbbm{1}_{(2,3)}\mathbbm{1}_{(1,3)}(\mu_2-\mu_1)^2 -  \mathbbm{1}_{(1,2)}\left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right)(\mu_1-\mu_2)^2 }}{\left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right)}\nonumber\\
    &\ \mu_3\geq \frac{\left(\mathbbm{1}_{(2,3)}\mu_2 + 
    \mathbbm{1}_{(1,3)}\mu_1\right) }{\left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right)}\nonumber\\
    &\ +\frac{ \sqrt{\epsilon\left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right) - \mathbbm{1}_{(2,3)}\mathbbm{1}_{(1,3)}(\mu_2-\mu_1)^2 -  \mathbbm{1}_{(1,2)}\left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right)(\mu_1-\mu_2)^2 }}{\left(\mathbbm{1}_{(2,3)} + 
    \mathbbm{1}_{(1,3)}\right)}\nonumber\\
\end{align}
The above equation leads to non-trivial bounds as $\epsilon$ satisfies equation~\eqref{eq:eps_big}. 

For the simple case of when edge $(2,3)$ is present and $(1,3)$ is not, the above analysis simplifies to,
\begin{align}
    \mu_2 - \sqrt{\epsilon - \mathbbm{1}_{(1,2)}(\mu_1 - \mu_2)^2}\leq \mu_3 \leq \mu_2 + \sqrt{\epsilon - \mathbbm{1}_{(1,2)}(\mu_1 - \mu_2)^2}
\end{align}
Similar analysis can be made when edge $(1,3)$ is present and $(2,3)$ is not. 

This shows that even with the complete knowledge of $\mu_1, \mu_2$ we can only estimate $\mu_3$ to a interval $[\mu_{\text{low}}, \mu_{\text{high}}]$ where the endpoints of interval are given by equation~\eqref{eq:bounds_simplified}. For the case when neither of the edges $(1,3)$ or $(2,3)$ are present (i.e. $\mathbbm{1}_{b,c} = 0$), then $\mu_3 \in [-\infty, \infty]$ even with the full knowledge of $\mu_1, \mu_2$ as there is no relation between the means of arm $3$ to arm $1,2$, this is also reflected in the equation~\eqref{eq:bounds_simplified}

\end{itemize}
In conclusion, with the linear bandit model $\mu_3$ was perfectly determined by the knowledge of $\mu_1, \mu_2$ wherelse with the graph bandit framework knowledge of $\mu_1, \mu_2$ could, at maximum, provide an interval $[\mu_{\text{low}}, \mu_{\text{high}}]$ in which value of $\mu_3$ exists, making the graph bandit framework far difficult to tackle. 

\begin{theorem}\label{thm:graph_vs_linear_thm}
Consider $n$-armed bandit setup parameterized by mean vector $\pmb{\mu}\in \mathbb{R}^n$. Let $D_{G, \epsilon}, D_{\pmb{\theta}}$ represent the subset of bandit problems in $\mathbb{R}^n$ as follows:
\begin{align}
    D_{G, \epsilon} &\ = \{\pmb{\mu}\in \mathbb{R}^n |~~ \langle \pmb{\mu}, L_G\pmb{\mu}\rangle \leq \epsilon, \epsilon>0\}\nonumber\\
    D_{\pmb{\theta}} &\ = \{\pmb{\mu}\in \mathbb{R}^n |~~\mu_i = \langle\mathbf{a}_i,\pmb{\theta}\rangle, ~~\mathbf{a}_i\in \mathbb{R}^k,~~\forall i\in [n]\}\nonumber
\end{align}
where $k < n, \pmb{\theta}\in \mathbb{R}^k$ indicates the reward vector and $L_G$ is the laplacian matrix corresponding to graph $G$. Then $D_{G, \epsilon} \not\subset D_{\pmb{\theta}}$, $D_{\pmb{\theta}} \not\subset D_{G, \epsilon}, m(D_{G, \epsilon}) >0$ and $m(D_{\pmb{\theta}})=0$ where $m(\cdot)$ is the Lebesgue measure on $\mathbb{R}^n$.
\end{theorem}

\textit{Sketch of proof :} We solidify the intuition from toy example~\ref{subsec:toy} to show the distinction in the two frameworks using measure theoretic argument. We split the $n$-armed bandit problem with graph side-information into two complementary scenarios:

(a) $L_{>}: \{\pmb{\mu}\in \mathbb{R}^n |~~ 0 < \langle \pmb{\mu}, L_G\pmb{\mu}\rangle \leq\epsilon, \epsilon> 0\}$

(b) $L_{=}:\{\pmb{\mu}\in \mathbb{R}^n |~~  \langle \pmb{\mu}, L_G\pmb{\mu}\rangle  = 0\}$

We prove that the set $D_{G, \epsilon} = L_{>}\cup L_{=}$ has fundamentally different measure theoretic properties than $D_{\pmb{\theta}}$ (linear bandits framework) and hence the two problems setups tackle completely different domain of questions. The complete discussion and full proof of Theorem~\ref{thm:graph_vs_linear_thm} can be obtained in Appendix~\ref{app:as_linear_bandit}

==> Content/Main_Resub_Arxiv/overview.tex <==
\begin{enumerate}
    \item Problem introduction
    \begin{itemize}
        \item Learning model
        \begin{itemize}
            \item $\sigma$-subgaussian noise
        \end{itemize}
        \item Graph smoothness 
        \begin{itemize}
            \item Laplacian 
            \item $\epsilon$-smooth
        \end{itemize}
        \item Goal of the paper
        \begin{itemize}
            \item Sampling algorithm
            \item Sample complexity for $\delta$-error
        \end{itemize}
    \end{itemize}
    \item Mean estimation
    \begin{itemize}
        \item Optimization formulation for $\hat{\pmb{\mu}}_T$
        \begin{itemize}
            \item Need strongly convexity for unique minima.
        \end{itemize}
        \item Cluster Identification
            \begin{itemize}
            \item Define $V(\{\pi_t\}_{i=1}^T,G), N(\{\pi_t\}_{t=1}^T), \mathbf{r}_T$ 
            \item Stub on $V(\{\pi_t\}_{t=1}^T, G) \succ 0$
            \item Algorithm
            \item Theoretical guarantee
        \end{itemize}
        \item closed form for $\pmb{\hat{\mu}}_T$
        \begin{itemize}
            \item Assumption on $\{\pi_t\}_{t=1}^T$ for $V(\{\pi_t\}_{t=1}^T, G) \succ 0$
            \item Lemma on closed form expression for $\hat{\pmb{\mu}}_T$
        \end{itemize}
    \end{itemize}
    \item Suboptimal arm elimination
    \begin{itemize}
        \item Variance estimation : Need to know how far is $\hat{\pmb{\mu}}$ from actual $\pmb{\mu}$ (with h.p.)
        \item Low prob. of "upper bound (best arm) < lower bound ($a_{\max}$)"
        \item Elimination routine
    \end{itemize}
    \item \textbf{GRUB} algorithm
    \begin{itemize}
        \item Sampling policy
        \begin{itemize}
            \item Cyclic
            \item Improved
        \end{itemize}
    \end{itemize}
    \item Sample complexity
    \begin{itemize}
        \item Minimum influence factor
        \begin{itemize}
            \item In a connected graph, sampling one influences confidence width of others
            \item Def of $d(\cdot,\cdot)$
            \item Existence of $d(\cdot, \cdot)$
            \item Nature of $\{t_i\}$ which generates $d(\cdot, \cdot)$\
            \item Independence of $d(\cdot, \cdot)$ from $T$.
        \end{itemize}
        \item Connection of $d(\cdot, \cdot)$ and confidence width $\|\mathbf{e}_i\|_{V_T^{-1}}$ decay rate.
        \begin{itemize}
            \item No sample regime.
            \item Low data regime.
            \item High data regime.
        \end{itemize}
        \item Subgraph class
        \begin{itemize}
        \item Ordering of graph
        \item Family of sub-graphs
        \end{itemize}
        \item Impact of $d(\cdot, \cdot)$ cause of removal of an edge in graph.
        \item Def of "bad" - arms inside a connected cluster $\mathcal{B}_i$.
        \item Sample complexity theorem for general graph G
        \item \td{Sample complexity result works for both sampling.}
        \item Specializations:
        \begin{itemize}
            \item Complete graph
            \item $\gamma$-expander to complete graph
        \end{itemize}
        \item $\epsilon -$ best arm identification
        \begin{itemize}
            \item \td{Inuition/ Discussion on this: within cluster its hard to decipher.}
            \item \td{Sample complexity result for $\epsilon-$best arm identification.}
        \end{itemize}
        \item Experiments:
        \begin{itemize}
            \item \td{Algorithms to compare : Cyclic, No-graph and proposed sampling}
            \item \td{Synthetic setup : 10 nodes each in 10 clusters. SBM graph p=1.0, q = $10^{-4}$}
            \item \td{Synthetic setup : Unequal nodes in 10 clusters. SBM graph p=1.0, q = $10^{-4}$}
            \item \td{Synthetic setup : 10 nodes each in 10 clusters. BA graph with m = 2}
            \item \td{Synthetic setup : Unequal nodes in 10 clusters. BA graph with m = 2}
            \item \td{Realistic graph}
        \end{itemize}
    \end{itemize}
\end{enumerate}

\subsection{Changelog}
\begin{itemize}
    \item $r^{i}_t \rightarrow r_{t, i}$
    \item $\mathcal{A} \rightarrow [n]$
\end{itemize}

==> Content/Main_Resub_Arxiv/special_cases.tex <==
\section{Special cases}

\subsubsection{Connection with vanilla $n$-armed bandit}

The main essence of Theorem

\begin{corollary}\label{cor:sample_complexity_star}
Consider the setup as in Theorem~\ref{thm: sample_complexity} with the further restriction that $G$ consists of a star subgraph with the central node as the optimal arm and $\Delta_i \leq 2\sqrt{\frac{2}{\rho\mathfrak{I}(i,F)}}\left(2\sigma\sqrt{14\log{\left(\frac{2a_0n\rho^2\mathfrak{I}(i, F)^2}{\delta}\right)}}\right)$, $\epsilon \leq \frac{c_0}{\rho}\log{\left(\frac{1}{\delta \Delta_{\min}}\right)}$ $\forall i\in [2, \dots, n]$. Define
\begin{align}
    T_{\text{sufficient}} \triangleq \sum_{i=2}^n \frac{1}{\Delta_i^2}\left[c_1\log\left(\frac{c_2}{\delta\Delta_i}\right)+\frac{\rho\epsilon}{2}\right]
\end{align}
Then, with probability at least $1-\delta$, \algoname{}: (a) terminates in no more than $T_{\text{sufficient}}$ rounds, and (b) returns the best arm $a^\ast = \arg\max_i \mu_i$.
\end{corollary}

\begin{comment}
\begin{corollary}[Star graph]\label{cor:sample_complexity_star}
Consider the setup as in Theorem~\ref{thm: sample_complexity} with the further restriction that $G$ consists of a star subgraph with the central node as the optimal arm and $\Delta_i \leq 2\sqrt{\frac{2}{\rho\mathfrak{I}(i,F)}}\left(2\sigma\sqrt{14\log{\left(\frac{2a_0n\rho^2\mathfrak{I}(i, F)^2}{\delta}\right)}}\right)$, $\epsilon \leq \frac{c_0}{\rho}\log{\left(\frac{1}{\delta \Delta_{\min}}\right)}$ $\forall i\in [2, \dots, n]$. Define
\begin{align}
    T_{\text{sufficient}} \triangleq \sum_{i=2}^n \frac{1}{\Delta_i^2}\left[c_1\log\left(\frac{c_2}{\delta\Delta_i}\right)+\frac{\rho\epsilon}{2}\right]
\end{align}
Then, with probability at least $1-\delta$, \algoname{}: (a) terminates in no more than $T_{\text{sufficient}}$ rounds, and (b) returns the best arm $a^\ast = \arg\max_i \mu_i$.
\end{corollary}
\end{comment}
In Corollary~\ref{cor:sample_complexity_star},  $T_{\text{sufficient}}$ is the same sample complexity as vanilla best arm identification, upto constant factors which is due to the fact that pulling one of the spoke arms does not yield much information about the other spoke arms, and this is the exact situation in the standard pure exploration setting.  



